Ontology without states: PBR as an argument for dynamics-first realism

The Pusey--Barrett--Rudolph (PBR) theorem is commonly taken to establish that a pure quantum state represents a physical property of the system to which it is assigned, rather than merely encoding knowledge. In this work, I distinguish between state-first and dynamics-first physical theories, and argue that this reading presupposes the former. These two types of theories support different approaches to causal explanation, and one of PBR's stated assumptions depends on the state-first approach. Using a recent interpretation of quantum theory as a concrete example, I show how a dynamics-first theory can explain the PBR correlations while maintaining a broadly epistemic reading of quantum states. I conclude that the PBR theorem supports a dilemma: either the quantum state is part of reality, or reality is not fundamentally built out of states.

==> old_pbr_section.tex <==
\section{The PBR theorem} \label{sec:pbr}

This section aims to provide a pedagogic and self-contained introduction to the PBR theorem. Since the theorem is usually understood as an argument in favour of wavefunction realism, it is natural to begin by considering what it would mean for the wavefunction to be \enquote{real}. 

The relevant version of wavefunction realism was pinned down in \citep{harrigan2010einstein} and is often called $\psi$\textit{-ontology}. The basic idea of $\psi$-ontology is that the wavefunction (up to global phase) of a system is a property of the physical state of the system. To refine this idea, we have to get clear on what we mean by a property of a physical state. 
To take a classical example, the energy of a system is a property of its physical state, but the probability distribution describing how likely the system is to have a given energy is not. 
The difference is that the energy of a system depends on nothing other than its physical state, whereas the probability of a system having a particular energy may depend on other contextual factors, such as the ensemble of which it is being considered as a member or the knowledge of the agent who assigns the distribution.
This suggests that $X$ should be regarded as a property of a physical state $\Lambda$ precisely if it is determined by $\Lambda$, so that we can think of $X$ as a function $X = f(\Lambda)$. 

Hence we can offer a more refined definition of $\psi$-ontology as the view that the wavefunction (up to phase) assigned to a system is uniquely determined by its physical state, $\psi = f(\Lambda)$. Put another way, no two phase-inequivalent wavefunctions are compatible with the same underlying physical state of the system.\footnote{Note that $\psi$-ontology does not imply that the wavefunction provides a complete description of the physical state of the system; it does not require that $\Lambda = g(\psi)$.
Indeed, the de Broglie-Bohm pilot-wave theory, which asserts that a system's state includes not only the wavefunction and corpuscles that it guides, is deemed $\psi$-ontic. $\psi$-ontology asserts that the wavefunction assigned to a system is property of its physical state, but it may be only one property among many.} 

What the PBR theorem shows is that, given some assumptions, $\psi$-ontology is true. This section will only explicitly derive a weaker version of the theorem, only ruling out physical states compatible with a pair of wavefunctions with a specific inner product, but which will nevertheless suffice for understanding the dynamics-first response to the full PBR theorem.

As with Bell's theorem, the bulk of PBR's argument makes no appeal to the specifics of quantum theory, and our presentation will emphasize this.
By considering an experimental scenario described in general operational terms, we will first show that a set of assumptions about how the observed statistics are explained at the ontological level collectively impose a constraint on those statistics. Quantum theory will come in only at the very end of the argument to derive a violation of the constraint, which will entail that at least one of the assumptions was false.

\subsection{Experiment and assumptions}

The setup of the relevant experiment is depicted in Figure \ref{fig:pbr_scenario}. Two systems are prepared using identical preparation devices and then fed into a device that measures the composite system. Beforehand, an agent at each preparation device chooses between two alternative procedures for preparing the system. We call these agents Alice and Bob.

\begin{figure}
    \centering
    \tikzfig{pbr_scenario}
    \caption{The experimental arrangement for the PBR scenario.}
    \label{fig:pbr_scenario}
\end{figure}

We assume that when Alice's device prepares the state of her system, the system ends up in some physical state $\lambda_{\bA} \in \Lambda_{\bA}$, and likewise that Bob's system ends up in some physical state $\lambda_{\bB} \in \Lambda_{\bB}$.
It is not easy to see what it would mean to deny this assumption, since it is compatible with the possibility that the systems have no physical properties at all, in which case the state would simply be trivial, i.e.\ $\Lambda_\bA = \Lambda_\bB = \{*\}$. 

The preparation procedures may not uniquely determine the physical state of the systems, but they are assumed to at least fix a probability distribution over physical states, meaning that each preparation device is characterized by a conditional probability distribution
\begin{equation}
    {\rm Prob}(\Lambda_{\bA}|S) \qquad \qquad {\rm and} \qquad \qquad {\rm Prob}(\Lambda_{\bB}|T),
\end{equation}
where $S \in \{0, 1\}$ and $T \in \{0, 1\}$ respectively denote the position Alice's and Bob's knobs, i.e.\ their chosen preparation settings.
Since Bob's and Alice's devices are constructed the same way, the two probability distributions are assumed to be equivalent (up to relabelling of the distributed variables),
\begin{equation} \label{eq:bob_isomorphism}
    {\rm Prob}(\Lambda_{\bA}|S)  \quad \cong \quad {\rm Prob}(\Lambda_{\bB}|T).
\end{equation}

For the sake of pedagogy, we will assume throughout that the physical state spaces takes only a finite number of possible values, i.e.\ $|\Lambda_\bA|, |\Lambda_\bB| \in \mathbb{N}$. However, none of the following arguments will crucially depend on this assumption. 

We now get on to the more substantive assumptions behind the theorem. The first will concern the overlap of the prepared probability distributions, the second and third will concern; way that the prepared systems combine to form a composite system; and the fourth will concern the way that physical states explain observed correlations. Our first assumption is that there is a state of Alice's system that can arise from either of the two preparation procedures.

\begin{assumption} \label{ass:epi}
    There exists a single physical state $\overline \lambda_{\bA}\in\Lambda_{\bA}$ of Alice's system that is compatible with both of her preparation procedures. By \cref{eq:bob_isomorphism}, it immediately follows that there exists an analogous state $\overline \lambda_{\bB}\in\Lambda_{\bB}$. Hence the assumption is that
\begin{equation} \label{eq:prep_non}
\begin{split}
      &\exists \overline \lambda_{\bA}\in\Lambda_{\bA}: \qquad   {\rm Prob}(\overline \lambda_{\bA} | S=0) \neq 0
    \quad {\rm and} \quad
    {\rm Prob}(\overline \lambda_{\bA} | S=1) \neq 0, \\
    {\rm and} \quad &
      \exists \overline \lambda_{\bB}\in\Lambda_{\bB}: \qquad   {\rm Prob}(\overline \lambda_{\bB} | T=0) \neq 0
    \quad {\rm and} \quad
    {\rm Prob}(\overline \lambda_{\bB} | T=1) \neq 0.
\end{split}
\end{equation}
\end{assumption}

(Although \cref{ass:epi} makes no mention of quantum states, note that if Alice's preparation procedures are interpreted as preparations of phase-inequivalent wavefunctions, then \cref{ass:epi} could be endorsed by a $\psi$-epistemologist but not a $\psi$-ontologist.)

Secondly, we assume that the composite system $\bA\bB$ has no holistic properties.
\begin{assumption} \label{ass:sup}
The joint physical state of the composite system $\bA\bB$ supervenes on the states of each subsystem; its physical state space is
\begin{equation}
\Lambda_{\bA \bB} = \Lambda_\bA \times \Lambda_\bB.
\end{equation}
\end{assumption}

In case this seems like a strong assumption, recall that in the present setting, $\bA$ and $\bB$ are prepared \textit{independently}, using different devices (and, if we like, at spacelike separation). For the PBR to go through, Assumption \ref{ass:sup} needs only hold in such situations.

The independence of the preparations also motivates the assumption that, for any pair of preparation procedures chosen by Alice and Bob, the resulting joint distribution over physical states factorizes.

\begin{assumption} \label{ass:prep}
The conditional probability distribution for the physical states of the two systems given pairs of settings factorizes, i.e.
\begin{equation} \label{eq:prep_independence}
{\rm Prob}(\Lambda_{\bA},\Lambda_{\bB}|S,T)
={\rm Prob}(\Lambda_{\bA}|S),{\rm Prob}(\Lambda_{\bB}|T).
\end{equation}
\end{assumption}

Only one assumption remains: the screening-off assumption discussed in the introduction.

\begin{assumption} \label{ass:screen}
The joint physical state \textit{screens off} any correlations between the preparation settings and the measurement outcome, i.e.
\begin{equation} \label{eq:screening_off}
{\rm Prob}\bigl(C\big|\Lambda_{\bA\bB},S,T\bigr)
=  {\rm Prob}\bigl(C\big|\Lambda_{\bA\bB}\bigr)
\end{equation}
\end{assumption}
The intuition here is that the outcome $C$ tells us no more about the choice of procedures $S$ and $T$ than what can already be inferred from what it tells us about the physical state $\Lambda_{\bA\bB}$. Or, put another way, Alice and Bob can only alter the outcome probabilities by altering the probabilities for the state $\Lambda_{\bA\bB}$.

\subsection{Deriving a constraint on observed statistics}

With our list of assumptions now complete, we use them to derive a constraint on the statistics of the observed variables $S$, $T$, and $C$. Specifically, we will prove the following.

\begin{lemma}
Assumptions \ref{ass:epi} -- \ref{ass:screen} imply that there exists an outcome $c \in C$ of Charlie's measurement that is compatible with all four possible pairs of settings:
\begin{equation} \label{eq:constraint}
\exists c\in C: \  \forall s\in S, t \in T, \qquad  {\rm Prob} (C= c| S=s, T=t)  >  0
\end{equation}
\end{lemma}

The strategy of the proof below is to show that there is some joint physical state $\tilde \lambda_{\bA\bB} = (\tilde \lambda_\bA, \tilde \lambda_\bB)$ that sometimes arises from each of the four pairs of preparation procedures, and that when this state does arise, no outcome can rule out any pair.

\begin{proof}
By \cref{ass:epi}, there exist physical states $\overline \lambda_\bA$ and $\overline \lambda_\bB$ that are attributed a nonzero probability by each associated preparation procedure, as expressed by Eq.\ \ref{eq:prep_non}. By \cref{ass:sup}, $\Lambda_\bA = \overline \lambda_\bA$ and $\Lambda_\bB = \overline \lambda_\bB$ if and only if $(\bA, \bB)$ is in the joint state $\overline \lambda_{\bA\bB} :=(\overline \lambda_\bA, \overline \lambda_\bB)$. By \cref{ass:prep}, this joint state $\overline \lambda_{\bA\bB}$ is compatible with each of the four pairs of settings; explicitly,
\begin{equation} \label{eq:join_comp}
\begin{split}
\forall s \in S, t\in T, \qquad
&{\rm Prob}(\Lambda_{\bA\bB} = \overline \lambda_{\bA\bB}\mid S=s,T=t)  \\
&= {\rm Prob}(\Lambda_{\bA} = \overline \lambda_{\bA}\mid S=s),{\rm Prob}(\Lambda_{\bB} = \overline \lambda_{\bB}\mid T=t) \\
& > 0.
\end{split}
\end{equation}
Now, whenever a measurement is performed, \textit{some} outcome has to arise, and thus there must be at least one measurement outcome compatible with $\overline \lambda_{\bA\bB}$; that is,
\begin{equation}
\exists c \in C: \qquad  {\rm Prob}(C=c|\Lambda_{\bA\bB} = \overline \lambda_{\bA\bB}) > 0.
\end{equation}
By \cref{ass:screen}, it follows from the last two equations that the conditional probability for this outcome $c$ given any pair of preparation settings is greater than $0$,
\begin{equation}
\begin{split}
&{\rm Prob}(C=c |S=s, T=t) \\
&= \sum_{\lambda_{\bA \bB} \in \Lambda_{\bA \bB}} {\rm Prob}(C=c |\Lambda_{\bA\bB} =  \lambda_{\bA\bB} ) {\rm Prob}(\Lambda_{\bA\bB} =  \lambda_{\bA\bB}|S=s, T=t) > 0.
\end{split}
\end{equation}
which is what we set out to prove.
\end{proof}

Since $S$, $T$, and $C$ are all observed events, the statistical constraint in \cref{eq:constraint} can be confirmed or refuted empirically. And if it is refuted, then we know that at least one of our assumptions is false.

==> qcmstuff.tex <==
\subsection{Explanation by causal mediators} \label{sec:general_explanation}

We will now show that more generally in DFQT, the explanatory strategy of showing that correlations arising from a fully mediated causal influence would not survive the counterfactual removal of the mediator is a successful one. 

We start by recapping some of the basics of the framework of quantum causal modelling \citep{Allen_2017, barrett2020quantum}. 
One of the main purposes of causal modelling is to predict the consequences of interventions on the systems $\{\bX_1,\ldots,\bX_n\}$  being investigated.
A local intervention on $\bX_i$ is represented by a \textit{quantum instrument}
\begin{equation}
    \mathcal I_{\bX_i{\bm \lambda}_i}^{K_i}
    =
    \left\{
        \mathcal I_{\bX_i{\bm \lambda}_i}^{k_i}
        \,\middle|\,
        k_i\in K_i
    \right\},
\end{equation}
where each $k_i \in K_i$ denotes a classical outcome of the intervention, and each $\mathcal I_{\bX_i{\bm \lambda}_i}^{k_i}$ is a completely positive map
\begin{equation}
    \mathcal I_{\bX_i{\bm \lambda}_i}^{k_i}
    :
    \bX_i^{\rm in}{\bm \lambda}_i
    \longrightarrow
    \bX_i^{\rm out}
\end{equation}
from an ingoing copy $\bX_i^{\rm in}$ of the system and an ancillary input ${\bm \lambda}_i$ to an outgoing copy $\bX_i^{\rm out}$ of the system. The sum $\sum_{k_i \in K_i}\mathcal I_{\bX_i{\bm \lambda}_i}^{k_i}$ of all maps in an instrument is required to be trace-preserving. A \textit{process operator} is a mathematical object that assigns probabilities to the outcomes of local interventions in a collection of quantum systems. Formally, a process operator $\sigma_{\bX_1\ldots\bX_n}$ is a multilinear map which, for any choice of local instruments and any joint state of their ancillary inputs, returns a joint probability distribution over the outcomes:
\begin{equation} \label{eq:process_operator_definition}
\sigma_{\bX_1\ldots\bX_n}: \quad 
\Big(
\mathcal I_{\bX_1{\bm \lambda}_1}^{K_1},\ldots,
\mathcal I_{\bX_n{\bm \lambda}_n}^{K_n};
\rho_{{\bm \lambda}_1\ldots{\bm \lambda}_n}
\Big)
\quad \longmapsto \quad 
p(K_1,\ldots,K_n).
\end{equation}
Thus a process operator specifies how the outcome statistics of local interventions are determined by the process connecting the systems. It is often represented instead by an operator using the Choi--Jamio{\l}kowski isomorphism \citep{choi1975completely, jamiolkowski1972linear}, but that representation is not needed here.

In the quantum causal modelling framework of \citep{barrett2020quantum}, a \textit{causal structure} is represented by a directed graph whose nodes are quantum systems and whose arrows represent noncommutation relations induced by the unitary dynamics (similar in spirit to how decoherence is defined in Dynamics-First Quantum Theory). A process operator is said to be \textit{compatible} with a causal structure when it can be recovered from an underlying unitary process that has that causal structure without introducing correlations between the modelled systems through initially correlated latent inputs. Theorem 4.10 of \citep{barrett2020quantum} establishes that a process operator is compatible with a given causal graph if and only if it satisfies the \textit{quantum Markov condition} for that graph. 

We are concerned only with a special corollary of the compatibility-Markovianity theorem, involving the causal graph
\begin{equation} \label{eq:causal_structure}
    \bX \quad \longrightarrow \quad \bY \quad \longrightarrow \quad \bZ,
\end{equation}
in which $\bY$ fully mediates the influence from $\bX$ to $\bZ$.
A tripartite process operator $\sigma_{\bX \bY \bZ}$ satisfies the quantum Markov condition for this graph if and only if $\sigma_{\bX \bY \bZ}$ admits a serial representation
\begin{equation} \label{eq:sequential_independence_form}
    \tikzfig{comb}
\end{equation}
for some channels $\cc_{\bX \rightarrow \bY}$ and $\cc_{\bY \rightarrow \bZ}$ and a state $\rho_\bX$.
Equivalently, the condition is that for some $\cc_{\bX \rightarrow \bY}$, $\cc_{\bY \rightarrow \bZ}$, and $\rho_\bX$,
\begin{equation}
    \sigma_{\bX \bY \bZ}(\ci_{\bX}^{K_\bX}, \ci_{\bY}^{K_\bY},  \ci_{\bZ}^{K_\bZ}) = {\rm Tr}\big(\ci_{\bZ}^{K_\bZ} \cc_{\bY \rightarrow \bZ} \ci_{\bY}^{K_\bY} \cc_{\bX \rightarrow \bY}\ci_{\bX}^{K_\bX}(\rho_{\bX}) \big)
\end{equation}
holds for arbitrary interventions $ \ci_{\bX}^{K_\bX}$, $ \ci_{\bY}^{K_\bY}$ and $ \ci_{\bZ}^{K_\bZ}$
 that do not involve ancillary systems. (The linear extension to a map on interventions with ancillaries is unique.) When this condition holds, we write $(\bX \bigCI_{\rm <} \bZ\mid \bY)_{\sigma_{\bX\bY\bZ}}$, and say that $\bX$ and $\bZ$ are \textit{sequentially independent} given $\bY$. The relevant corollary of the compatibility-Markovianity theorem is that $\sigma_{\bX\bY\bZ}$ is compatible with causal structure $\bX \rightarrow \bY\rightarrow \bZ$ precisely if the sequential independence relation $(\bX \bigCI_{\rm <} \bZ\mid \bY)_{\sigma_{\bX\bY\bZ}}$ holds.

In turn, the sequential independence relation $(\bX \bigCI_{\rm <} \bZ\mid \bY)_{\sigma_{\bX\bY\bZ}}$ implies that if the intervention at $\bY$ carries no information from $\bY^{\rm in}$ to $\bY^{\rm out}$, then there will be no correlation between the outcomes of interventions on $\bX$ and $\bZ$. Indeed, if the intervention at $\bY$ is a trace-and-replace channel that discards the ingoing system and prepares the outgoing system in some new state, $\mathcal T_{\bY}^{\rho}(\cdot):=\rho_{\bY}^{\rm out}{\rm Tr}_{\bY^{\rm in}}(\cdot)$, then for any $ \ci_{\bX}^{K_\bX}$ and $ \ci_{\bZ}^{K_\bZ}$, the distribution over $K_\bX$ and $K_\bZ$ factorizes, $p(K_\bX,K_\bZ)=p(K_\bX) p(K_\bZ)$. 

We now come to the implications of this result for causal explanation in DFQT. In DFQT, process operators serves as useful tools for predicting both the probabilities of events in the actual scenario, and probabilities in counterfactual scenarios in which the dynamics are modified. In the PBR example, the process operator ${\sigma_{\bS\bT\bA\bB\bO}}$ represented by
\begin{equation} \label{eq:pbr_process_operator}
    \tikzfig{pbr_proc_op},
\end{equation} 
can be used to predict the actual probabilities arising in our PBR model given that ${\color{red} D^\downarrow}={\color{red} 0} $ and ${\color{red} E^\downarrow}={\color{red} 0}$. Indeed, by inserting the density operators $\ket 0 \bra 0_\bD$ and $\ket 0 \bra 0_\bE$, we have effectively conditioned on ${\color{red} D^\downarrow}={\color{red} 0}$ and ${\color{red} E^\downarrow}={\color{red} 0}$ (and by inserting maximally mixed states at $\bS^{\rm in}$ and $\bT^{\rm in}$, we have not conditioned on any facts about these systems).
As a result, interventions of the form $\{\pi_{{\bX}}^{{\color{blue} x^\uparrow}}\epsilon_{{\bX}}^{{\color{red} x^\downarrow}}(\cdot)
\epsilon_{{\bX}}^{{\color{red} x^\downarrow}}
\pi_{\bX}^{{\color{blue} x^\uparrow}}|({\color{red} x^\downarrow}, {\color{blue} x^\uparrow}) \in {\color{red} X^\downarrow} \times {\color{blue} X^\uparrow}\}$ associated with the emergent events at $\bS$, $\bT$, $\bO$, $\bA$ and $\bB$ recover the PBR correlations exactly. But ${\sigma_{\bS\bT\bA\bB\bO}}$ can also be used to predict the probabilities for the counterfactual scenario where the causal connection at $\bA \bB$ is broken. These counterfactual probabilities are predicted in precisely the same way as the actual ones, except that at $\bA$ and $\bB$ we insert interventions $\ct_\bA^{I/d}$ and $\ct_\bB^{I/d}$ that trace and replace with the maximally mixed state. 

Given the operational consequence of sequential independence noted above, it follows, via the compatibility-Markovianity theorem, that the loss of setting-outcome correlations in the counterfactual PBR scenario can be derived from the compatibility of  ${\sigma_{\bS\bT\bA\bB\bO}}$ with the causal structure $\bS\bT \rightarrow \bA\bB \rightarrow \bO$. 

More generally, whenever a process operator $\sigma_{\bX \bY \bZ}$ accurately predicts both the actual DFQT probabilities and those resulting from counterfactual modifications to the circuit, the compatibility of $\sigma_{\bX \bY \bZ}$ with the causal structure $\bX \rightarrow \bY \rightarrow \bZ$ implies that there would have been no correlations between events emerging at $\bX$ and $\bZ$ had the causal connection at $\bY$ been broken, and hence that it is the mediating role of $\bY$ that explains those correlations in the actual scenario. 

Hence shifting from a state-first to a dynamics-first ontology does not mean abandoning causal explanation, but only changing how one is given. While it is only in state-first theories that one can show that a system's mediating role is responsible for correlations by demonstrating that its state screens off those correlations, in dynamics-first theories one can still demonstrate this by showing that the correlation does not survive a counterfactual break in the causal connection. The classical causal modelling framework of \citep{spirtes2000causation, pearl2009causality} implies that complete causal mediators satisfy a screening-off assumption, but the quantum dynamics-first theory of DFQT is more at home in the quantum causal modelling framework of \citep{Allen_2017, barrett2020quantum}, which implies instead that they satisfy sequential independence. 

